MoSAIC: Aligned Intervention Supervision for Part-Local Motion Style Transfer

Editing character motion often requires transferring a gesture or gait from one or more reference motions while preserving the source action, timing, root trajectory, and unselected body regions. Existing motion datasets, however, rarely provide paired targets for arbitrary part-local content--reference combinations, and self-reconstruction training may allow a diffusion model to reproduce the content motion while underusing the routed reference. We present MoSAIC, a latent diffusion framework for part-local reference-conditioned motion style transfer. MoSAIC factorizes content and reference features by anatomical region, preserves the root trajectory through a separate conditioning pathway, and routes user-selected references to individual body parts. Its central contribution is aligned intervention supervision, which constructs synchronized references and counterfactual targets through controlled local transformations, making both the requested regional response and the motion to be preserved directly observable during training. In a frozen evaluation comprising 128 motions and 896 routed conditions, part-masked routing reduces preserved-region error from 70.64 to 66.45~mm and matched-noise off-target leakage from 18.08 to 9.88~mm relative to whole-body routing, while retaining a positive selected-region response. A matched-budget continuation study further shows that retaining aligned intervention supervision produces an 8.8\% relative increase in selected-target response and a 2.0-percentage-point increase in requested-route influence concentration. These results demonstrate that MoSAIC improves the response--preservation trade-off required for selective and controllable part-local motion editing.

==> legacy/04-experiments-pre-reorganization.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate four questions: whether the selected model retains HumanML3D
generation quality, where it lies on the whole-body content--style frontier,
whether masked routing improves local response without unnecessary change,
and which qualitative behaviors and limitations remain.

\subsection{Experimental Protocol}

\noindent\textbf{Selection and inference.}
HumanML3D \cite{guo2022generating} provides disjoint training, validation, and
test identifier sets.  Training and aligned-pair construction use only the
training split.  We select epoch 189 by minimum validation FID (0.2953), then
evaluate the frozen checkpoint on the test split.  The primary inference
setting is fixed at zero-style classifier-free guidance \(s=2.0\), 50-step
DDIM sampling, and \(\eta=0\).  The final training seed is 1234.  Earlier
architecture development was informed by previous HumanML3D test and CMU
observations; the final estimates are therefore development-aware rather than
results from previously untouched benchmarks.
For HumanML3D, H-FID measures distribution distance in the standard
text--motion evaluator, R-precision measures retrieval agreement, and
diversity measures pairwise generated-embedding distance.  These metrics
evaluate the base generator but are not style-transfer endpoints.

\noindent\textbf{Whole-body protocols.}
We follow the public MCM-LDM CMU evaluation \cite{song2024mcmldm}.  Style
recognition accuracy (SRA), trajectory style inconsistency (TSI), and
foot-sliding factor (FSF) use a fixed grid of 900 ordered content--reference
pairs.  Content recognition accuracy (CRA) and Fr\'echet motion distance
(FMD) use a separate 1,600-pair grid.  SRA and CRA are top-1 classifier
accuracies; FMD is computed in the content-classifier feature space.  Higher
SRA and CRA and lower FMD, TSI, and FSF are preferred.  The checkpoint,
primary guidance, pair order, evaluator assets, and generation seed were
frozen before this final evaluation.

\noindent\textbf{Part-local protocol.}
Our principal locality benchmark contains 128 deterministically selected
HumanML3D test motions and seven aligned interventions per motion, yielding
896 routed conditions.  Each condition restores identical initial diffusion
noise for the content-style control \(Y_0\), whole-body route
\(Y_{\mathrm{full}}\), masked route \(Y_M\), and wrong-route control.  Pose
distances are measured on root-aligned joints.  If \(\mathcal C\) is the set
of joints changed by the exact counterfactual \(X_M\), selected-target
improvement is
\begin{equation}
 \mathrm{STI}=1-
 \frac{d_{\mathcal C}(Y_M,X_M)}
 {d_{\mathcal C}(Y_0,X_M)+\epsilon}.
 \label{eq:sti}
\end{equation}
Preserved-region error (PRE) measures the distance from \(Y_M\) to the
factual motion on unchanged joints; causal off-target leakage (COL) measures
the matched-noise distance from \(Y_M\) to \(Y_0\) there; and exact
counterfactual error (ECE) measures whole-motion distance to \(X_M\).
Higher STI and lower PRE, COL, and ECE are preferred.
The wrong-route control sends the changed source condition to a predeclared
unrelated region, testing whether improvement depends on the anatomical
assignment rather than merely exposing the model to a reference.  The same
matched outputs produce a six-by-six influence matrix whose rows are requested
routes and columns are measured regions.  Since a terminal head rotation
changes orientation without necessarily moving its joint position, head
position STI is undefined; we report a separately labelled post-hoc
rotation-space supplement.

HumanML3D test values are means with 95\% confidence intervals over 20 fixed
sampling seeds from one trained model.  For the aligned benchmark, 95\%
intervals use 10,000 content-motion-clustered bootstrap resamples; paired
route tests use Wilcoxon statistics with Holm correction.  The fixed-seed CMU
reports do not retain sample-level classifier decisions, so we make no paired
significance claim against published baselines.  Full configuration and
metric definitions appear in Appendix~\ref{app:experiment_details}.
The robustness subsets are frozen before evaluation: three sampling seeds use
the first 32 motions, while two unseen intervention magnitudes use the first
64.  These subsets do not alter the primary 896-condition estimate.

\subsection{Generation and Whole-Body Transfer}

\begin{table}[t]
\centering
\caption{Validation selection and disjoint HumanML3D test generation quality.
Test values are means \(\pm\) 95\% confidence intervals over 20 sampling
seeds from the validation-selected model.}
\label{tab:humanml_final}
\begingroup
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrrr@{}}
\toprule
Split & H-FID $\downarrow$ & R@1 (\%) $\uparrow$ & R@2 (\%) $\uparrow$ &
R@3 (\%) $\uparrow$ & Div.\\
\midrule
Validation & 0.2953 & 47.21 & 66.56 & 77.26 & 9.205\\
Test & $0.3077{\pm}0.0032$ & $45.32{\pm}0.23$ &
$64.35{\pm}0.28$ & $74.70{\pm}0.27$ & $9.174{\pm}0.071$\\
\bottomrule
\end{tabular*}
\endgroup
\end{table}

Table~\ref{tab:humanml_final} asks whether intervention training has damaged
the underlying generator.  HumanML3D FID (H-FID) changes from 0.2953 on
validation to \(0.3077\pm0.0032\) on the disjoint test split, while
text--motion R-precision and embedding diversity remain stable across
sampling seeds.  This excludes gross generator collapse.  These retrieval
metrics assess text-conditioned generation, however, and do not measure
reference-style transfer.
The small validation-to-test H-FID change is also important procedurally:
model selection used the validation loader, whereas all reported test
replications were generated only after the checkpoint and inference setting
were frozen.

\begin{table}[t]
\centering
\caption{Whole-body transfer on the MCM-LDM CMU protocol. Baselines are
published values; \mosaic uses the frozen primary setting. The comparison is
not a seed-matched reproduction.}
\label{tab:sota}
\begingroup
\footnotesize
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrrr@{}}
\toprule
Method & SRA (\%) $\uparrow$ & CRA (\%) $\uparrow$ & FMD $\downarrow$ &
TSI $\downarrow$ & FSF $\downarrow$\\
\midrule
1DConv+AdaIN~\cite{aberman2020unpaired} & 57.00 & 31.18 & 42.68 & 0.2200 & 2.0500\\
STGCN+AdaIN~\cite{park2021diverse} & 17.66 & \textbf{60.43} & 129.44 & \textbf{0.1100} & 0.9300\\
Motion Puzzle~\cite{jang2022motionpuzzle} & 46.33 & 26.31 & 113.31 & 0.2200 & 2.4300\\
MCM-LDM~\cite{song2024mcmldm} & \textbf{58.00} & 35.75 & \textbf{27.69} & 0.4000 & 1.2800\\
\midrule
\mosaic & 50.33 & 38.13 & 39.88 & 0.5020 & \textbf{0.8285}\\
\bottomrule
\end{tabular*}
\endgroup
\end{table}

The CMU experiment instead asks where the selected checkpoint lies on the
whole-body style--content frontier.  At \(s=2.0\), \mosaic obtains 50.33\%
SRA and 38.13\% CRA (Table~\ref{tab:sota}).  Relative to the published
MCM-LDM point, it retains more classifier-measured content but has weaker
style recognition and worse FMD.  Its lower FSF does not overturn the weaker
style and feature-distance results.  The comparison therefore documents a
different operating point, not state-of-the-art whole-body transfer, and
does not evaluate anatomical routing.
Because the published baseline rows are neither regenerated with matched
noise nor available as sample-level predictions, differences in this table
are descriptive rather than paired statistical comparisons.

\subsection{Part-Local Counterfactual Evaluation}
\label{sec:partlocal_quant}

\begin{table}[t]
\centering
\caption{Aligned evaluation on 128 test motions and 896 conditions. Errors
are root-aligned millimeters. Position STI excludes 128 head conditions,
whose intervention changes terminal-joint orientation only.}
\label{tab:partlocal_primary}
\begingroup
\footnotesize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Control & STI $\uparrow$ & PRE $\downarrow$ & COL $\downarrow$ & ECE $\downarrow$\\
\midrule
Content style $Y_0$ & 0.000 & \textbf{64.84} & \textbf{0.00} & 81.80\\
Whole body $Y_{\mathrm{full}}$ & \textbf{0.215} & 70.64 & 18.08 & 81.42\\
\textbf{Masked $Y_M$} & 0.198 & 66.45 & 9.88 & \textbf{78.24}\\
Wrong route & -0.290 & 106.03 & 84.65 & 127.11\\
\bottomrule
\end{tabular*}
\endgroup
\end{table}

The principal question is whether selecting only the requested source regions
improves the response--preservation balance.  Whole-body routing produces the
largest selected response, but also modifies regions that the exact target
preserves.  Masked routing reaches STI 0.198 and improves aggregate ECE by
3.56\,mm relative to \(Y_0\).  Relative to whole-body routing, it reduces PRE
by 4.19\,mm and matched-noise COL by 8.20\,mm
(Table~\ref{tab:partlocal_primary}).  The wrong-route control degrades every
primary metric, confirming that the anatomical source assignment matters.
The result supports selective response rather than exact preservation.
The motion-clustered interval for masked STI is [0.178, 0.217].  The ECE
improvement has interval [3.18, 3.91]\,mm; reductions relative to whole-body
routing are [3.83, 4.55]\,mm for PRE and [7.86, 8.54]\,mm for COL.  These
paired estimates support the aggregate balance claim, while the route-wise
results below show that the benefit is not uniform across anatomy.

\begin{table}[t]
\centering
\caption{Masked response by requested route over 128 motions. P-STI uses
joint positions; supplemental R-STI uses articulation-joint rotation because
the terminal head intervention is position-invisible.}
\label{tab:partlocal_routes}
\begingroup
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrr@{}}
\toprule
Route & P-STI $\uparrow$ & R-STI $\uparrow$ & COL (mm) $\downarrow$\\
\midrule
Spine & 0.142 & 0.179 & 11.99\\
Head & -- & \textbf{0.346} & 7.02\\
Left arm & 0.090 & 0.190 & \textbf{6.76}\\
Right arm & 0.065 & 0.235 & 9.70\\
Left leg & 0.335 & 0.103 & 8.75\\
Right leg & \textbf{0.413} & 0.163 & 12.98\\
\bottomrule
\end{tabular*}
\endgroup
\end{table}

Response varies substantially by anatomy.  Position response is strongest
for the legs and spine and remains positive but weaker for both arms
(Table~\ref{tab:partlocal_routes}).  A supplemental SO(3) geodesic measure
makes the terminal head rotation observable, yielding R-STI 0.346; because it
was introduced after identifying the structural blind spot of position STI,
it is supporting rather than primary evidence.  All five
position-identifiable routes have positive bootstrap intervals, although
statistical detectability should not be confused with uniformly strong
transfer.
In particular, arm P-STI values of 0.090 and 0.065 are far below the leg
values of 0.335 and 0.413.  The supplemental head R-STI interval is
[0.289, 0.400], but its post-hoc status limits the strength of the associated
claim.

The matched-noise influence matrix places 42.4\% of total response on its
requested-route diagonal, compared with 16.7\% under uniform influence.  This
concentration indicates selective but incomplete anatomical isolation:
spine interventions, in particular, propagate into the head and arms through
the kinematic chain.  The full matrix and route-wise uncertainty are reported
in Appendix~\ref{app:full_local_results}.  On frozen subsets, STI has
between-sampling-seed standard deviation 0.005 and remains positive at
unseen \(0.75\times\) and \(1.25\times\) intervention magnitudes.  These checks
vary sampling noise and controlled transformation strength, not training
initialization or natural style.
Masked root-trajectory error changes only from 0.3342\,m for \(Y_0\) to
0.3353\,m, and contact F1 changes from 0.9485 to 0.9477.  These auxiliary
results are consistent with retained global motion structure, although they
do not imply framewise equality outside the route.

\subsection{Qualitative Results and Guidance Behavior}
\label{sec:qualitative_routing}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/results/part_local_transfer_joints.png}
\caption{\textbf{Part-local routing.}
Rows assign hands-high style to the arms, open-leg style to the legs, and
old-motion style to the spine. Columns show content, reference, whole-body
transfer, and selected-part transfer. Content, reference, and initial noise
are matched within each row at the primary setting. The selected examples
illustrate routing behavior rather than population-level selectivity.}
\label{fig:part_local_transfer}
\end{figure*}

Figure~\ref{fig:part_local_transfer} provides matched-input comparisons for
arms, legs, and spine.  Changing the source map changes the requested
anatomical chain while retaining the content and trajectory source.  The
weaker visible arm response is consistent with the quantitative route
analysis, but these selected sequences do not measure leakage rates.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/results/multi_reference_composition_joints.png}
\caption{\textbf{Two-reference source assignment.}
Circular-walk content is followed by hands-high and open-leg references,
single-route controls, and their composition. Matched generated panels use
the same initial noise. The composed route assigns the references to arms and
legs while retaining content conditions elsewhere. This selected case
demonstrates the inference interface, not population-level composition
generalization.}
\label{fig:multi_reference_composition}
\end{figure*}

Figure~\ref{fig:multi_reference_composition} assigns one reference to both
arms and another to both legs in a single denoising run; the head and spine
retain content-derived conditions.  The output remains a coherent circular
walk and exhibits both routed cues, although the arm cue is attenuated.
This establishes simultaneous source assignment for the displayed case, not
a quantitative multi-reference success rate.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/results/guidance_sweep_joints.png}
\caption{\textbf{Guidance behavior.}
The same content, two routed references, and initial noise are held fixed as
guidance increases from \(s=2.0\) to \(s=3.25\). Each panel overlays ordered
poses. The response changes gradually; only \(s=2.0\) is the predeclared
primary setting, and the remaining panels are frozen-checkpoint sensitivity
diagnostics.}
\label{fig:guidance_visual}
\end{figure*}

Increasing guidance raises SRA while reducing CRA, and FMD improves only up
to an intermediate scale before worsening.  Figure~\ref{fig:guidance_visual}
shows the corresponding gradual qualitative change under matched noise.
No scale dominates all metrics, so \(s=2.0\) remains the primary operating
point; the complete sweep is in Appendix~\ref{app:guidance}.
Auxiliary aligned diagnostics show that masked trajectory error and contact
F1 remain close to \(Y_0\), while the full numerical results are reported in
Appendix~\ref{app:auxiliary}.
Across the frozen sweep, SRA rises from 50.33\% to 60.78\% as CRA falls from
38.13\% to 32.75\%; FMD reaches its minimum at \(s=2.75\).  The sweep
therefore describes an inference-time frontier rather than identifying a
replacement primary result.

\subsection{Limitations}

The evidence comes from one independently trained final model.  We have not
performed equal-compute local retraining of Motion Puzzle, MoST, or MCM-LDM,
and therefore do not claim superiority over those methods for part-local
transfer.  The exact locality benchmark uses controlled synthetic
interventions rather than natural-reference part-local targets, and no human
perceptual study is available.  Arm response remains weaker than leg and
spine response, while the influence matrix shows incomplete anatomical
isolation.  Two-reference composition is demonstrated qualitatively but lacks
a frozen population-level benchmark.  The sampling-seed study does not
measure variation across training seeds.  Finally, earlier development was
informed by HumanML3D test and CMU observations.  The results consequently
support controlled part-local response and preservation under the aligned
protocol, not natural-style or population-level multi-reference
generalization.

\FloatBarrier


==> legacy/experiment-details-pre-reorganization.tex <==
\section{Experimental Details}
\label{app:experiment_details}

\subsection{Full Training and Inference Configuration}

HumanML3D is represented by 22 joints and 263 rotation-invariant features at
20\,fps.  After the released mirroring augmentation, the local split files
contain 23,384 training, 1,460 validation, and 4,384 test identifiers; these
are processed identifiers rather than unique source motions.  Their pairwise
overlap is zero.  Training motions are restricted to 40--196 frames.

The selected run was continued from the earlier temporal-injection checkpoint
and trained through epoch 200 with early stopping disabled.  Six NVIDIA L40S
GPUs processed 64 motions each, giving global batch size 384.  Of 326.01\,M
parameters, 27.42\,M were trainable.  AdamW used a fixed learning rate of
\(10^{-5}\) and seed 1234.  After a 20-epoch curriculum, batches contained
75\% factual self-denoising rows and 25\% aligned same-motion intervention
rows; no arbitrary unpaired row was used.  Factual rows sampled all 1,000
diffusion steps, while intervention rows sampled \(t\in[0,400)\).  The
scaled-linear DDPM schedule used
\(\beta_1=8.5{\times}10^{-4}\) and \(\beta_{1000}=0.012\).

The diffusion objective weight was 1.0.  Weights for selected-part response,
unselected-part preservation, style-code matching, source margin, root,
contact, velocity, decorrelation, and descriptor matching were respectively
0.025, 0.05, 0.0125, 0.0125, 0.05, 0.0125, 0.025, 0.0025, and 0.025.
Inference used 50 DDIM steps, \(\eta=0\), zero-style guidance, and primary
scale \(s=2.0\).  HumanML3D test evaluation used seeds 1234--1253.  CMU and
the primary aligned evaluation used seed 1234.

The CMU style grid contains \(30\times30=900\) ordered pairs from six style
classes; the content/realism grid contains \(40\times40=1,600\) pairs from
eight content classes.  The checkpoint, sampler, two-worker mapping, ordered
pair lists, evaluators, and asset digests were frozen in evaluation manifests
before final generation.  The aligned suite fixes 128 test motions by
identifier hash and applies seven conditions per motion: two spine, one head,
two arm, and two leg interventions.  The first 32 motions define the
sampling-seed subset and the first 64 define the intervention-magnitude
subset.

\subsection{Metric Definitions}

\begin{table}[t]
\centering
\caption{Definitions, evaluation populations, and preferred directions of
reported metrics. Feature distances are measured in the corresponding learned
evaluator space.}
\label{tab:metrics}
\begingroup
\footnotesize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{\columnwidth}{@{}l>{\raggedright\arraybackslash}Xcc@{}}
\toprule
Metric & Definition & Unit / \(N\) & Direction\\
\midrule
SRA & Top-1 target-style classification of transferred motion
    & \% / 900 & \(\uparrow\)\\
CRA & Top-1 source-content classification of transferred motion
    & \% / 1,600 & \(\uparrow\)\\
FMD & Fr\'echet distance between real and generated content-classifier features
    & feature distance / 1,600 & \(\downarrow\)\\
TSI & Mean per-frame horizontal root-path error to content
    & m / 900 & \(\downarrow\)\\
FSF & Two-foot horizontal displacement accumulated below 5\,cm
    & m per motion / 900 & \(\downarrow\)\\
H-FID & Fr\'echet distance in the HumanML3D text--motion evaluator
    & feature distance & \(\downarrow\)\\
R@1 & Top-1 HumanML3D text--motion retrieval precision
    & \% & \(\uparrow\)\\
Div. & Mean pairwise distance between generated motion embeddings
    & feature distance & target-matched\\
STI & Changed-joint target-error reduction relative to matched \(Y_0\)
    & ratio / 768 & \(\uparrow\)\\
PRE & Error to factual motion on exact unchanged joints
    & mm / 896 & \(\downarrow\)\\
COL & Matched-noise change from \(Y_0\) on exact unchanged joints
    & mm / 896 & \(\downarrow\)\\
ECE & Whole-motion error to the exact aligned counterfactual
    & mm / 896 & \(\downarrow\)\\
\bottomrule
\end{tabularx}
\endgroup
\end{table}

The changed set contains joints whose factual-to-counterfactual displacement
exceeds 1\,mm; its complement defines preserved joints.  The primary
position-only STI is undefined for the 128 head-nod conditions because a
terminal-joint rotation need not displace that joint.  R-STI is a post-hoc
supplement based on SO(3) geodesic error at the intervention articulation
joint.  It does not replace position STI.

HumanML3D confidence intervals summarize 20 fixed generation seeds from one
training run.  The aligned intervals use 10,000 bootstrap resamples clustered
by content motion.  Route-wise comparisons use two-sided paired Wilcoxon
tests with Holm correction over the six routes and paired standardized mean
differences.  CMU uses one fixed generation seed over each full grid.  The
external aggregate reports do not contain per-example classifier decisions,
precluding paired bootstrap comparisons with published methods.

\subsection{Guidance Sensitivity}
\label{app:guidance}

\begin{table}[t]
\centering
\caption{Frozen-checkpoint CMU guidance sweep. The dagger marks the
predeclared primary setting; all other rows are secondary sensitivity
measurements on identical ordered grids.}
\label{tab:cfg}
\begingroup
\footnotesize
\setlength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}crrrrr@{}}
\toprule
Scale & SRA (\%) $\uparrow$ & CRA (\%) $\uparrow$ & FMD $\downarrow$ &
TSI $\downarrow$ & FSF $\downarrow$\\
\midrule
2.00$^\dagger$ & 50.33 & 38.13 & 39.88 & 0.5020 & 0.8285\\
2.25 & 55.11 & 36.44 & 38.62 & 0.5053 & 0.8214\\
2.50 & 58.11 & 35.13 & 37.84 & 0.5086 & 0.8151\\
2.75 & 59.89 & 34.13 & 37.49 & 0.5116 & 0.8095\\
3.00 & 60.67 & 33.56 & 37.56 & 0.5144 & 0.8087\\
3.25 & 60.78 & 32.75 & 38.00 & 0.5169 & 0.8071\\
\bottomrule
\end{tabular*}
\endgroup
\end{table}

Increasing \(s\) from 2.00 to 3.25 raises SRA by 10.44 percentage points and
reduces CRA by 5.38 points.  FMD reaches its minimum of 37.49 at \(s=2.75\)
and then worsens, whereas TSI increases monotonically and FSF decreases.  At
\(s=2.50\), SRA is 0.11 points above the published MCM-LDM result, but CRA is
0.63 points lower and FMD remains 10.15 higher.  No sensitivity row dominates
all metrics or replaces the predeclared \(s=2.0\) result.

\subsection{Sampling-Seed and Intervention-Magnitude Robustness}

\begin{table}[t]
\centering
\caption{Masked-routing robustness subsets. Seed rows use 32 motions and all
seven conditions; magnitude rows use 64 motions. Only sampling noise or
intervention strength changes.}
\label{tab:partlocal_robustness}
\begingroup
\footnotesize
\setlength{\tabcolsep}{2.8pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Variant & STI $\uparrow$ & PRE $\downarrow$ & COL $\downarrow$ & ECE $\downarrow$\\
\midrule
Seed 1234 & 0.230 & 54.46 & 9.10 & 66.80\\
Seed 1235 & 0.224 & 54.90 & 8.98 & 67.93\\
Seed 1236 & 0.220 & 57.15 & 8.92 & 69.31\\
\quad between-seed SD & 0.005 & 1.44 & 0.09 & 1.26\\
\midrule
\(0.75\times\) magnitude & 0.187 & 58.65 & 7.29 & 68.11\\
\(1.25\times\) magnitude & 0.228 & 60.02 & 11.86 & 74.91\\
\bottomrule
\end{tabular*}
\endgroup
\end{table}

Response remains positive under both unseen intervention magnitudes.  The
stronger intervention increases STI but also COL and ECE, exposing the
response--preservation trade-off.  The seed rows vary only diffusion sampling
noise for one trained model and therefore do not establish training-seed
robustness.

\subsection{Auxiliary Trajectory, Contact, and Sliding Diagnostics}
\label{app:auxiliary}

\begin{table}[t]
\centering
\caption{Auxiliary aligned diagnostics at the primary setting. A-FID uses
HumanML3D evaluator features against exact targets; the exact target row is
an oracle reference, not model output.}
\label{tab:aligned_auxiliary}
\begingroup
\footnotesize
\setlength{\tabcolsep}{2.8pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Control & A-FID $\downarrow$ & Traj. (m) $\downarrow$ &
Contact F1 $\uparrow$ & Slide (m) $\downarrow$\\
\midrule
Content style $Y_0$ & 0.3984 & 0.3342 & 0.9485 & 1.1535\\
Whole body $Y_{\mathrm{full}}$ & 0.3592 & 0.3358 & 0.9473 & 1.1236\\
\textbf{Masked $Y_M$} & 0.3780 & 0.3353 & 0.9477 & 1.1450\\
Wrong route & 3.6021 & 0.5285 & 0.9132 & 1.6852\\
Exact target $X_M$ & 0.0000 & 0.0000 & 1.0000 & 0.8634\\
\bottomrule
\end{tabular*}
\endgroup
\end{table}

Masked routing keeps trajectory error and contact F1 close to the
content-style control and improves A-FID from 0.3984 to 0.3780.  Whole-body
routing obtains lower A-FID and sliding but causes more off-target change in
Table~\ref{tab:partlocal_primary}.  The wrong route degrades every diagnostic,
showing why global distribution quality cannot replace explicit locality
measurement.

\subsection{Full Influence and Uncertainty Results}
\label{app:full_local_results}

\begin{table}[t]
\centering
\caption{Matched-noise influence matrix in root-aligned millimeters. Rows are
requested routes and columns are measured regions; bold entries form the
requested-route diagonal.}
\label{tab:partlocal_influence}
\begingroup
\scriptsize
\setlength{\tabcolsep}{1.7pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
\toprule
Request & Sp. & Hd. & L-A & R-A & L-L & R-L\\
\midrule
Spine & \textbf{17.72} & 39.86 & 28.73 & 31.93 & 13.77 & 13.42\\
Head & 2.07 & \textbf{34.71} & 7.54 & 6.35 & 6.60 & 6.84\\
Left arm & 2.68 & 6.35 & \textbf{27.35} & 8.54 & 5.97 & 5.27\\
Right arm & 4.22 & 9.75 & 12.18 & \textbf{30.82} & 8.56 & 8.91\\
Left leg & 2.08 & 5.03 & 7.31 & 7.37 & \textbf{75.78} & 11.84\\
Right leg & 2.81 & 6.78 & 10.47 & 10.07 & 16.55 & \textbf{117.56}\\
\bottomrule
\end{tabular*}
\endgroup
\end{table}

\begin{table}[t]
\centering
\caption{Route-wise position-STI uncertainty. Intervals use
motion-clustered bootstrap resampling; \(p_{\mathrm H}\) is the
Holm-corrected paired Wilcoxon result against \(Y_0\).}
\label{tab:partlocal_significance}
\begingroup
\footnotesize
\setlength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrr@{}}
\toprule
Route & P-STI [95\% CI] $\uparrow$ & \(p_{\mathrm H}\) & \(d_z\)\\
\midrule
Spine & 0.142 [0.128, 0.155] & \(2.81{\times}10^{-21}\) & 1.817\\
Left arm & 0.090 [0.061, 0.120] & \(1.40{\times}10^{-6}\) & 0.527\\
Right arm & 0.065 [0.033, 0.096] & \(7.21{\times}10^{-5}\) & 0.353\\
Left leg & 0.335 [0.297, 0.372] & \(5.52{\times}10^{-21}\) & 1.541\\
Right leg & 0.413 [0.366, 0.459] & \(2.28{\times}10^{-20}\) & 1.532\\
\bottomrule
\end{tabular*}
\endgroup
\end{table}

All five position-identifiable routes have positive intervals and remain
detectable after family-wise correction.  The arm responses and paired effect
sizes are nevertheless substantially smaller than those of the spine and
legs.  For the supplemental orientation endpoint, head R-STI is 0.346 with a
motion-bootstrap 95\% interval of [0.289, 0.400].  The influence diagonal
contains 42.4\% of total response; large spine-to-head and spine-to-arm terms
show that anatomical isolation remains incomplete.

